SynergyNet: Bridging the Gap between Discrete and Continuous Representations for Precise Medical Image Segmentation

In recent years, continuous latent space (CLS) and discrete latent space (DLS) deep learning models have been proposed for medical image analysis for improved performance. However, these models encounter distinct challenges. CLS models capture intricate details but often lack interpretability in terms of structural representation and robustness due to their emphasis on low-level features. Conversely, DLS models offer interpretability, robustness, and the ability to capture coarse-grained information thanks to their structured latent space. However, DLS models have limited efficacy in capturing fine-grained details. To address the limitations of both DLS and CLS models, we propose SynergyNet, a novel bottleneck architecture designed to enhance existing encoder-decoder segmentation frameworks. SynergyNet seamlessly integrates discrete and continuous representations to harness complementary information and successfully preserves both fine and coarse-grained details in the learned representations. Our extensive experiment on multi-organ segmentation and cardiac datasets demonstrates that SynergyNet outperforms other state of the art methods, including TransUNet: dice scores improving by 2.16%, and Hausdorff scores improving by 11.13%, respectively. When evaluating skin lesion and brain tumor segmentation datasets, we observe a remarkable improvement of 1.71% in Intersection-over Union scores for skin lesion segmentation and of 8.58% for brain tumor segmentation. Our innovative approach paves the way for enhancing the overall performance and capabilities of deep learning models in the critical domain of medical image analysis.

==> sections/prework.tex <==
\section{Related Work}
\subsection{Continuous Latent Space Models} 
Continuous latent space(CLS) models have gained significant popularity in the field of medical image segmentation. These models offer a flexible and powerful framework for capturing the complex and continuous variations present in medical images. Existing work can be divided into CNNs, transformers, and hybrid models. \\

\textbf{CNN-based CLS models:}
Convolutional Neural Networks (CNNs) have emerged as the widely accepted standard for various computer vision applications. Image segmentation, a task that involves assigning class labels to individual pixels, has particularly benefited from the effectiveness of CNNs. Initial work in the field of image segmentation, such as Fully Convolutional Networks (FCN)\cite{long2015fully}, and SegNet\cite{badrinarayanan2017segnet}, demonstrated the effectiveness of CNNs in this domain. FCN eliminated the need for fully connected layers and enabled pixel-wise segmentation. SegNet, on the other hand, introduced an encoder-decoder architecture that utilized pooling indices for efficient upsampling. Other notable work consist of DeepLab\cite{chen2017deeplab}, \cite{noh2015learning},\cite{zhao2017pyramid} which improves FCNs by increasing the receptive field and capturing contextual information. CNN models have also achieved remarkable success in medical imaging tasks, notably with the introduction of U-net\cite{hatamizadeh2022unetr}, which inspired subsequent research on U-shaped encoder-decoder architectures\cite{zhou2018unetpp,cai2020dense,huang2020unet,oktay2018attention}. Notably, studies\cite{cai2020dense,huang2020unet,cai2020dense} have explored enhancing the encoder-decoder structure with dense skip connections, leading to improved performance in diverse medical domains. Furthermore, encoder-decoder arch. have also shown great success in Semi-SL\cite{you2022class,you2022mine,you2023action++,you2023bootstrapping,you2023implicit,you2023rethinking}\\

\textbf{Multi-head Cross-attention Mechanism}
 emerges as a pivotal convergence point in both natural language processing (NLP) and computer vision domains, amalgamating the potency of multi-head attention and cross-attention mechanisms. It combines the strengths of multi-head attention, which is rooted in the Transformer model's mechanism for focusing on different parts of input, and cross-attention, which extends this capability to interactions between different data types. For instance, in tasks like image captioning and understanding relationships between images and text, the concept proves its utility. This innovation has led to improvements in machine translation, question answering, and text summarization as well, showcasing its potential to revolutionize the handling of diverse data. In our study, we harness Multi-Head Cross Attention to jointly model discrete and continuous latent spaces, capturing complementary fine and coarse-grained information. This is particularly critical in medical image segmentation, underscoring its significance.

\textbf{Transformer-based CLS models}
Vision transformers\cite{dosovitskiy2020image} and their variants\cite{ruan2022vision,liu2021swin,yuan2021tokens,xia2022vision,lin2017feature} have emerged as powerful models in computer vision, akin to the remarkable success of transformers in Natural Language Processing (NLP). These models leverage self-attention mechanisms to learn global information and have achieved impressive results in various visual tasks such as object classification\cite{yuan2021tokens}, segmentation\cite{chen2021TransUNet,cao2022swin,lin2017feature}, and detection\cite{zhu2020deformable,cai2016unified}. Their end-to-end solutions demonstrate the versatility and effectiveness of vision transformers across different vision domains. For instance, Swin Transformer\cite{liu2021swin} introduces a hierarchical vision transformer that efficiently computes self-attention locally using a shifted windowing approach. CrossViT\cite{chen2021crossvit} proposes a dual-branch vision transformer followed by a cross-attention module, enabling richer feature representations while maintaining linear time complexity. These approaches have proven effective in improving performance. In addition to fully transformer-based models, recent methods like Swin-UNet\cite{cao2022swin} and TransUNet\cite{chen2021TransUNet} adopt pure transformer architectures with a U-shaped design based on Swin Transformer for 2D segmentation tasks. More recent work such as FCT\cite{tragakis2023fully} and Transwnet\cite{10097129} more accurately capture local and global information and improve medical segmentation performance.  \\

\textbf{Hybrid CLS models}
Hybrid models combine the capabilities of CNN and transformers models to capture local and global complementary features tackling the limitation of each. TransUNet\cite{chen2021TransUNet} combines the strengths of both CNNs and transformers\cite{graham2022transformer} to capture both low-level and high-level features, while UNETR\cite{hatamizadeh2022unetr} utilizes a transformer-based encoder and a CNN-based decoder for 3D segmentation tasks. More recent approach HiFormer \cite{heidari2023hiformer}effectively incorporates both global and local information and utilizes a
novel transformer-based fusing scheme to maintain feature
richness and consistency for the task of 2D medical image
segmentation.
 
\subsection{Discrete Latent Space models}

\textbf{Vector Quantization}
Vector quantization is a classical method for compressed coding that employs a codebook and quantization strategy. Typically using mean square error (MSE), it identifies similar patterns in the codebook to replace original input data. It's akin to discrete representation learning, using a one-hot vector coefficient. Research\cite{gray1984vector, mao2021discrete, santhirasekaram2022vector} demonstrates its impact on visual understanding and model robustness. Notably, VQVAE\cite{van2017neural} leverages a codebook-based neural network for effective discrete feature distribution learning in images, widely adopted in generative models. In our study, we integrate VQVAE's discrete representation with continuous representation, enhancing medical image segmentation.

Discrete latent space (DLS) models have emerged as a promising approach in various domains, including computer vision and natural language processing. Unlike continuous latent space models, which utilize continuous variables, DLS models leverage discrete variables to represent latent features or concepts. However, the application of DLS in medical image segmentation remains an active and evolving research domain. For instance, Gangloff et al. \cite{gangloff2022leveraging} exploit DLS techniques for anomaly detection, while Jin et al. \cite{jin2022deep} employ a DLS-based model \cite{van2017neural} as a regularizer for semantic segmentation of fundus retina images. Pinaya et al. \cite{pinaya2022unsupervised} introduce VQUnet, a DLS-based approach for 3D anomaly detection and segmentation in brain imaging. Additionally, Santhirasekaram et al. \cite{santhirasekaram2022vector} demonstrate the robustness and interpretability of vector quantization in semantic segmentation tasks. These studies collectively contribute to the ongoing exploration and advancement of DLS methods in the context of medical image segmentation.

\section{Model's Parameters Analysis:} We compare the parameter count of SynergyNet (131.82M), UNet (147.81M), and VQUNet (131.56M), indicating that SynergyNet achieves competitive representation capacity while potentially offering comprehensibility and capturing fine-grained details.

\section{Limitations:}
While SynergyNet has demonstrated success, it can also be susceptible to issues inherited from its quantizer module, including limited scalability and sensitivity to hyperparameters. Additionally, relying solely on a strategy that selects the most similar codebook item to represent input might face limitations in capturing intricate data patterns, potentially leading to information loss. In cases like ACDC, where fixed ROIs require segmentation, continuous space can offer a more viable option due to vector quantization's structured sparsity property. Furthermore, we observe that CLS and DLS models experience false negatives due to poor inter-class dependencies, a problem partially addressed by SynergyNet. As a result, there is merit in conducting further research on SynergyNet. 


